Fast and Secure Decentralized Optimistic Rollups Using Setchain

Modern blockchains face a scalability challenge due to the intrinsic throughput limitations of consensus protocols. Layer 2 optimistic rollups (L2) are a faster alternative that offer the same interface in terms of smart contract development and user interaction. Optimistic rollups perform most computations offchain and make light use of an underlying blockchain (L1) to guarantee correct behavior, implementing a cheaper blockchain on a blockchain solution. With optimistic rollups, a sequencer calculates offchain batches of L2 transactions and commits batches (compressed or hashed) to the L1 blockchain. The use of hashes requires a data service to translate hashes into their corresponding batches. Current L2 implementations consist of a centralized sequencer (central authority) and an optional data availability committee (DAC). In this paper, we propose a decentralized L2 optimistic rollup based on Setchain, a decentralized Byzantine-tolerant implementation of sets. The main contribution is a fully decentralized "arranger" where arrangers are a formal definition combining sequencers and DACs. We prove our implementation correct and show empirical evidence that our solution scales. A final contribution is a system of incentives (payments) for servers that implement the sequencer and data availability committee protocols correctly, and a fraud-proof mechanism to detect violations of the protocol.

==> algorithms/challenges.tex <==
\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small logger.}
    \label{logger}
    \small
    \begin{algorithmic}[1]
  	\State  \textbf{Init:} $proposedBatchTags = \emptyset$
	\hspace{2em} $confirmedBatchTags = []$ 
        \State $stakers = []$ \hspace{2em} $challenges = \emptyset$
        \hspace{2em} $challengeId = 0$
        \State $arrangerProcessesPKs = ??????$
        \Function{post}{$id, h, sigs$}
          \State \<assert> $isArrangerProcess(sender)$
          \State \<assert> $ isValidStake(value)$
          \State $proposedBatchTags \leftarrow proposedBatchTags \cup
          (id, h, sigs)$
          \State $stakers[(id,h,sigs)] \leftarrow stakers[(id,h,sigs)]
          \cup \{sender\}$ \Comment{save poster for rewards.}
        \EndFunction
        \Function{confirmBatch}{$id, h, sigs$}
          \State \<assert> $ is??????(sender)$
          \State $proposedBatchTags \leftarrow proposedBatchTags \setminus
          \{(id, h, sigs)\}$
          \State $confirmedBatchTags[id] = (h,sigs)$
          \State $returnStakes(id,h,sigs)$
          \State $rewardArrangerProcesses(id,h,sigs)$ 
        \EndFunction
        \Function{stake}{$id, h, sigs$}
          \State \<assert> $ isValidStake(value)$
          \State \<assert> $ (id,h,sigs) \in proposedBatchTags$
          \State $stakers[(id,h,sigs)] \leftarrow stakers[(id,h,sigs)]
          \cup \{sender\}$ 
        \EndFunction

        \Function{removeBatch}{$id,h,sigs,client$}
          \State \<assert> $(id,h,sigs) \in proposedBatches$        
          \State  $proposedBatchTags \leftarrow proposedBatchTags \setminus
          \{(id, h, sigs)\}$
          \State $stakers[(id,h,sigs)] \leftarrow \emptyset$
          \State $rewardClient(client,TODO)$ \Comment{VER: cuanto le
            mandamos? depende del numero de stakers? o si se juega
            contra uno solo a la vez, depende del numero de pasos que
            se jugaron?}
        \EndFunction
        
        \Function{initDataChallenge}{$id, h, sigs, staker$}  
          \State \<assert> $ enoughTokens(value, type)$
          \State \<assert> $ staker \in stakers[(id,h,sigs)]$
          \Comment {tambien hay q chequearlo cuando da los datos?}
          \State \<assert> $ notInActiveChallenge(staker)$
          \State $deadline \leftarrow now() + challengeDuration$
          \State $challenged \leftarrow staker$
          \State $challenger \leftarrow sender$
          \State $challenge[challengeId] \leftarrow (challenger,
          challenged, deadline, active, h)$
          \State $challengeId \leftarrow challengeId++$
        \EndFunction
        \Function{DataChallenge}{$challengeId, compressedBatch$}  
          \State \<assert> $ isDataChallenge(challengeId)$
          \State \<assert> $ active == state(challengeId)$
          \State \<assert> $ sender = challenges[challengeId].turn$
          \State $batch = brotli.Decompress(compressedBatch)$
          \If{$\hash(batch) == hash(challengeId)$}
            \State $setWinner(challengeId, challenged)$
          \Else
            \State $setWinner(challengeId, challenger)$
          \EndIf
        \EndFunction
        \Function{SignatureChallenge}{$id,h,sigs$}
          \State \<assert> $(id,h,sigs) \in proposedBatches$
          \State \<assert> $value >= SignatureChallengeCost$
          \If{$|sigs| < f+1$ or $!validSignature(arrangerProcessesPKs,
            id,h, sigs)$}
            \State $removeBatch(id,h,sigs,sender)$
           \EndIf 
        \EndFunction
        
        \Function{ValidityChallenge}{$id,h,sigs,e,proof$}
          \State \<assert> $(id,h,sigs) \in proposedBatches$
          \State \<assert> $value >= ValidityChallengeCost$
          \If{$validProof(e,proof,h)$ and $validElement(e)$}
            \State $removeBatch(id,h,sigs,sender)$
          \EndIf  
        \EndFunction

        \Function{IntegrityChallenge}{$id1,h1,sigs1,e,proof1, id2, proof2$}
          \State \<assert> $(id1,h1,sigs1) \in proposedBatches$        
          \State \<assert> $value >= IntegrityChallengeCost$
          \State $(h2,\_) \leftarrow confirmed[id2]$
          \If{$validProof(e,proof1,h1)$ and $validProof(e,proof2,h2)$}
            \State $removeBatch(id1,h1,sigs1,sender)$
          \EndIf
        \EndFunction

        \Function{validProof}{$e,proof,root$}
          \State $n \leftarrow \hash(e)$
          \For{$(b,h) \in proof$}
            \If{$b$}
              \State $n \leftarrow \hash(n ++ h)$
            \Else
              \State $n \leftarrow \hash(h ++ n)$
            \EndIf  
          \EndFor
          \State \<return> $n == root$
        \EndFunction
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/client-seqDC-opt.tex <==
\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small Optmisitc client protocol for Arranger with a
      centralized Sequencer and Data Committee.} 
    \label{alg:client-seqDC-opt}
    \small
    \begin{algorithmic}[1]
  	\Function{\<ArrangerApi>.\<Add>}{$t$}
          \State \<SequencerApi>.\<Add>(t)
        \EndFunction
        \Function{\<ArrangerApi>.\<Translate>}{$(id,h,\textcolor{red}{sigs(id,h)})$}
                  \State $\<notContacted> \leftarrow \{ p :
                  sig_p(id,h) \in sigs(id,h)\}$
          \While{not received $b$ such that $\hash(b) == h$ and
            $|\<notContacted>| > 0$}
            \State take $p$ from $\<notContacted>$
            \State \<call> $p$.\<Translate>$(h)$
            \State $\<notContacted> \leftarrow \<notContacted>
            \setminus \{p\}$

          \EndWhile 
          \State \<wait> for response $b$ such that $\hash(b) == h$
          \State \<return> $b$
        \EndFunction
         
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


==> algorithms/client-seqDC.tex <==
\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small Correct clients protocol (Sequencer + DAC).}
    \label{alg:client-seqDC}
    \small
    \begin{algorithmic}[1]
  	\Function{\<ArrangerApi>.\textnormal{\<add>}}{$t$}
          \State \<SequencerApi>.\<add>(t)
          \State \<return>
        \EndFunction
        \Function{\<ArrangerApi>.\textnormal{\<translate>}}{$\textit{id},h$}
          \ForAll{ \(p\) is a DAC member} $p$.\<translate>$(\<id>,h)$
          \EndFor
          \State \<wait> for one response $b$ with $\hash(b) == h$
          \State \<return> $b$
        \EndFunction
    \end{algorithmic}
    % \begin{algorithmic}[1]
  	% \Function{\<ArrangerApi>.\<Add>}{$t$}
    %       \State \<SequencerApi>.\<Add>(t)
    %       \State \<return>
    %     \EndFunction
    %     \Function{\<ArrangerApi>.\<Translate>}{$(id,h)$}
    %       \State $\<notContacted> \leftarrow \{ p : p \text{ is a DAC member}\}$
    %       \While{(not received $b$ with  $\hash(b) == h$) and $|\<notContacted>| > 0$}
    %         \State take $p$ from $\<notContacted>$
    %         \State \<call> $p$.\<Translate>$(h)$
    %         \State $\<notContacted> \leftarrow \<notContacted>
    %         \setminus \{p\}$
    %       \EndWhile
    %       \State \<wait> for one response $b$ with $\hash(b) == h$
    %       \State \<return> $b$
    %     \EndFunction
    % \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/client-setchain-opt.tex <==
\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small Optmisitc client protocol for Arranger built on
      top of Setchain.} 
    \label{alg:client-setchain-opt}
    \small
    \begin{algorithmic}[1]
  	\Function{\<ArrangerApi>.\<Add>}{$t$}
          \State \<call> \<Add>$(t)$ in 1 server.
        \EndFunction
        \Function{\<ArrangerApi>.\<Translate>}{$(id,h,sigs(id,h))$}
          \While{not received $b$ such that $\hash(b) == h$ and there
              is a server $i$ with  $sig_i(id,h) \in sigs(id,h)$ not
              contacted yet}
              \State \<call> $i.\<Translate>(id,h)$
          \EndWhile 
          \State \<wait> for response $b$ such that $\hash(b) == h$
          \State \<return> $b$
        \EndFunction
         
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


==> algorithms/client-setchain.tex <==
\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small Correct client protocol for Arranger implemented
      on top of Setchain.}
    \label{alg:client-setchain}
    \small
    \begin{algorithmic}[1]
  	\Function{\<ArrangerApi>.\<Add>}{$t$}
          \State \<call> \<Add>$(t)$ in $f+1$  servers.
        \EndFunction
        \Function{\<ArrangerApi>.\<Translate>}{$id,h$}
          \While{not received $b$ such that $\hash(b) == h$ and there
              are servers not contacted yet}
            \State \<call> \<Translate>$(id,h)$ in a server not
            contacted before
          \EndWhile
          \State \<wait> for response $b$ such that $\hash(b) == h$
          \State \<return> $b$
        \EndFunction
         
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


==> algorithms/payment-client.tex <==

\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small API and algorithm for a client that pay for the
      translation of a hash.}
    \label{alg:sequencer}
    \small
    \begin{algorithmic}[1]

    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/payment-server.tex <==

\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small API and algorithm for server that charges for the
      translation of a hash.}
    \label{alg:sequencer}
    \small
    \begin{algorithmic}[1]
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> algorithms/recorder.tex <==
\begin{figure}[t!]
  \begin{algorithm}[H]
    \caption{\small Recorder.}
    \label{recorder}
    \small
    \begin{algorithmic}[1]
  	\State  \textbf{Init:} $SetchainServers$
	\hspace{2em} $L1Contract$ 
        \Function{GetEpochHashAndSignatures}{$h$}
        \State $sigs \leftarrow \emptyset$
        \While{true}
          \State $\text{pick } s \text{ from }  SetchainServers$
          \State $(S,H,\_) \leftarrow s.Get()$ \Comment{podriamos modificar la API de Setchain para que tenga algo como getEpochSigs(h) que devuelva (E,\{sign(hash(h,E))\}}
          \State $E \leftarrow H(h)$
          \State $hash\_E \leftarrow hash(<<h,E>>)$
          \State $sigs[hash\_E] \leftarrow sigs[hash\_E] \cup \{s : s = sign_i(hash\_E) \wedge \exists epoch\_signature(h,s) \in S \cup H \}$
          \If{ | sigs[hash\_E] | == f + 1}
             \State \<return> $(hash(E), sigs[hash\_E])$
          \EndIf     
         \EndWhile
         \EndFunction
     \Function{PostBatch}{}
       \State $h \leftarrow L1Contract.LastBatchNumber() + 1$
       \State $(hash,sigs) \leftarrow GetEpochHashAndSignatures(h)$
       \State \<return> $L1Contract.PostBatch(h,hash,sigs)$
       \Comment{capaz habria que juntar todas las firmas? En anytrust usan BLS.. ver bien esto!}
     \EndFunction    
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


==> algorithms/sequencer-frontrunning.tex <==
\begin{figure}[b!]
  \begin{algorithm}[H]
    \caption{\small Centralized Sequencer that does front-running.}
    \label{alg:sequencer-frontrunning}
    \small
    \begin{algorithmic}[1]
  	\State \textbf{init: } $\<allTxs> \leftarrow \emptyset $, 
        $\<pendingTxs> \leftarrow \epsilon$,  $\<batchId>
        \leftarrow 0$ 
        \Function{add}{$t$}
          \State \ldots \Comment{Same as
            lines~\ref{seq-add}-\ref{seq-add-allTxs} in Alg.~\ref{alg:sequencer}}
          \State \textit{\<inform> Malicious client \texttt{C} about
            transaction t} \label{alg:seq-frontrunning-inform}
          \State \Return
        \EndFunction
        \Upon{\<timetopost>}
        % \When{$|pendingTxs| == \<maxSize>$ or \textit{timeout}(\(\<maxTime>\))}
          \State $b \leftarrow rearrangeTxs(\<pendingTxs>)$ \label{alg:seq-frontrunning-rearrange}
          \State \ldots \Comment{Same as
            lines~\ref{seq-when-hash-b}-\ref{seq-when-end} in Alg.~\ref{alg:sequencer}}
        \EndUpon  
        % \EndWhen
    \end{algorithmic}
  \end{algorithm}
  \vspace{-2em}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/latex/preamble.tex <==
\pdfobjcompresslevel0

\usepackage[T1]{fontenc}
\usepackage[tt=false, type1=true]{libertine} 
\usepackage[varqu]{zi4}
\usepackage[libertine]{newtxmath}
\usepackage{amssymb}
\usepackage{algorithm}
\usepackage{algpseudocode}


